Effect of null aether field on weak deflection angle of black holes

We study the light rays in a static and spherically symmetric gravitational field of null aether theory (NAT). To this end, we employ the Gauss-Bonnet theorem to compute the deflection angle by a NAT black hole in the weak limit approximation. Using the optical metrics of the NAT black hole, we first obtain the Gaussian curvature and then calculate the leading terms of the deflection angle. Our calculations show how gravitational lensing is affected by the NAT field. We also show once again that the bending of light stems from a global and topological effect.

==> observables.tex <==
\section{\added{Observables}}
\added{Gravitational lensing observables including positions, magnifications and differential time delays between lensed images. Here, we focus on the observational relevance (positions, magnifications and differential time delays between lensed images) of the results which is derived in the previous sections. The corresponding lens equation (or ray-tracing equation) with the angular positions
of the images ($\theta$), and the actual position of the source ($\beta$) shown in Fig. 1 is as follows \cite{keeton1,keeton2}:}
 
\begin{figure}
\centering
\color{blue}
\includegraphics[width=10cm]{obs.png}
\caption{\label{ipda}Lens geometry.}
\end{figure}

\begin{equation}
\tan \beta =\tan \theta -D\ \left[ \tan \theta +\tan (\hat{\alpha}-\theta )%
\right] 
\end{equation}
\added{where $D$ is the ratio of the distance from the lens to the source, $d_{LS}$ and the distance from the observer to the source, $d_S$: $%
D\equiv d_{LS}/d_{S}$.
Then, in weak lens approximation ($
\alpha D_{s} \simeq \hat{\alpha} D_{d s}
$), the above lens equation ($\beta=\theta-\frac{D_{d s}}{D_{s}} \hat{\alpha}(\theta)$) for  black hole with Einstein angle $\theta_{E}$, is calculated as follows:}

\begin{equation}
\beta=\theta-\frac{\theta_{\mathrm{E}}^{2}}{\theta},\label{lens}
\end{equation}
\added{where the impact parameter, $
u=D_{d} \theta  $, and the Einstein angle (for the position consistent with $\beta= 0$) is} \begin{equation}
\theta_{\mathrm{E}}=\sqrt{\frac{4 M D_{\mathrm{LS}}}{D_{\mathrm{L}} D_{\mathrm{S}}}},\label{Eangle}
\end{equation}
\added{and the Einstein radius} \begin{equation}
R_{E}=\theta_{E} D_{d}.
\end{equation}
\added{Using the Einstein angle \ref{Eangle} in \ref{lens}, we get $
\beta \theta=\theta^{2}-\theta_{E}^{2}
$. Then corresponding angular position of images are obtained as follows:} \begin{equation}
\theta_{\pm}=\frac{1}{2}[\beta \pm \sqrt{\beta^{2}+4 \theta_{\mathrm{E}}^{2}},
\end{equation} \added{and  the angular separation between the two images are}
 \begin{equation}
 \Delta \theta=\theta_{+}-\theta_{-}=\sqrt{\beta^{2}+4 \theta_{\mathrm{E}}^{2}}.
 \end{equation}
\added{Magnification $\mu \left( \theta \right) $ of images takes place
because the bending of light by the lens focuses more light rays from the
source into a solid angle at the observer brightening up the image. It is
defined by} %
\begin{equation}
\mu \left( \theta \right) =\left[ \frac{\sin \beta }{\sin \theta }\frac{%
d\beta }{d\theta }\right] ^{-1},
\end{equation}
 \added{and the magnification for the black hole is calculated as follows:} \begin{equation}
\mu_{\pm}=\frac{\beta^{2}+2 \theta_{\mathrm{E}}^{2}}{2 \beta \sqrt{\beta^{2}+4\theta_{\mathrm{E}}^{2}}} \pm \frac{1}{2}.
\end{equation}

\added{Moreover one can calculate the total flux of the images (with the original flux of the source  $F_{\mathrm{src}}$), using the magnifications as follows:}
\begin{equation}
\begin{aligned} F_{\mathrm{tot}} &=\left(\mu_{+}+\mu_{-}\right) F_{\mathrm{src}} \\ &=\frac{\beta^{2}+2 \theta_{\mathrm{E}}^{2}}{\beta \sqrt{\beta^{2}+4 \theta_{\mathrm{E}}^{2}}} F_{\mathrm{src}}. \end{aligned}
\end{equation}


\added{The last important observable for the weak gravitational lensing is the time delay which can be calculated using the following equation:}
\begin{equation}
T=\int_{R_{\mathrm{src}}}^{r_{0}} \frac{\mathrm{d} t}{\mathrm{d} r} \mathrm{d} r+\int_{r_{0}}^{R_{\mathrm{obs}}} \frac{\mathrm{d} t}{\mathrm{d} r} \mathrm{d} r,
\end{equation}
where \begin{equation}
\frac{\mathrm{d} t}{\mathrm{d} r}=\frac{\sqrt{f(r)^{-1} r^2 f(r_0)}}{f(r) \sqrt{r_{0}} \sqrt{\frac{r^2}{r_0} \frac{f(r_0)}{f(r)}-1}},
\end{equation}
 \added {and using $
u=D_{\mathrm{L}} \sin \theta
$ the corresponding differential time delay for the black hole is obtained as follows:}


 \begin{equation*}
\Delta T= T_{+}-T_{-}
\end{equation*}
\begin{equation}
\begin{array}{l}{=4 M\left[\frac{\beta}{2 \theta_{\mathrm{E}}^{2}} \sqrt{\beta^{2}+4 \theta_{\mathrm{E}}^{2}}\right.} {\left.+\ln \left(\frac{\sqrt{\beta^{2}+4 \theta_{\mathrm{E}}^{2}}+\beta}{\sqrt{\beta^{2}+4 \theta_{\mathrm{E}}^{2}}-\beta}\right)\right]}.\end{array}
\end{equation}

\added{The angular position of images for the homogeneous magnetized plasma is}

\begin{equation}
\theta=\frac{1}{2}(\beta \pm \sqrt{\beta^{2}+4 \Theta_{\pm}^{2}})
\end{equation} with
\begin{equation}
\Theta_{\pm}=\theta_{E} \sqrt{\frac{1}{2}\left[1+\left(1-\frac{\omega_{e}^{2}}{\omega_{\infty}^{2}}\right)^{-1}\right]}.
\end{equation}
\added{Hence, using the above angular position and repeated the calculation, it is found that the presence of the plasma causes a shift of the angular position of images \cite{keeton1,keeton2,keeton, XEr,BK11,Turimov}. }


